Determination of X-Ray Transient Source Positions By Bayesian Analysis of Coded Aperture Data

We present a new method of transient point source deconvolution for coded-aperture X-Ray detectors. Our method is based upon the calculation of the likelihood function and its interpretation as a probability density for the transient source position by an application of Bayes' Theorem. The method obtains point estimates of source positions by finding the maximum of this probability density, and interval estimates of prescribed probability by choosing suitable contours of constant probability density. We give the results of simulations that we performed to test the method. We also derive approximate analytic expressions for the predicted performance of the method. These estimates underline the intuitively plausible properties of the method and provide a sound quantitative basis for the design of coded-aperture systems.

==> README <==
%auto-ignore
This paper will appear in the Proceedings of the RIKEN Workshop on
All-sky X-ray Observations in the Next Decade.  It uses a set of LATEX
macros provided (RIKEN2A.sty, WORKSHOP.sty, psbox.sty) provided by the
conference organizers.  One of these macros apparently generates two
errors at the \maketitle command in the text when compiled using
LATEX2e.  No error is produced if compiled with LATEX209.  The LATEX2e
compilation will go through to the end if you just type a carriage
return at each of the two error messages, producing the correct DVI
file.

Sorry about that,

Carlo Graziani
c-graziani@uchicago.edu

